Forces and fluctuations in planar, spherical and tubular membranes

Lipid membranes constitute very particular materials: on the one hand, they break very easily under microscopical stretching; on the other hand, they are extremely flexible, presenting deformations even at small scales. Consequently, a piece of membrane has an area excess relative to its optically resolvable area, also called projected area. From a mechanical point of view, we can thus identify three tensions associated to lipid membranes: the mechanical effective tension $\tau$, associated to an increase in the projected area and to the flattening of the fluctuations; the tension $\sigma$, associated to the microscopical area of the membrane and thus non measurable, but commonly used in theoretical predictions; and its macroscopical counterpart measured through the fluctuation spectrum, $r$. Up to now, the equality between these quantities was taken for granted when analyzing experimental data. In this dissertation, we have studied, using the projected stress tensor, whether and under which conditions it is justified to assume $\tau = \sigma$. We studied three geometries (planar, spherical and cylindrical) and obtained the relation $\tau \approx \sigma - \sigma_0$, where $\sigma_0$ is a constant depending only on the membrane's high frequency cutoff and on the temperature. Accordingly, we conclude that neglecting the difference between $\tau$ and $\sigma$ is justifiable only to membranes under large tensions: in the case of small tensions, corrections must be taken into account. We have studied the implications of this result to the interpretation of experiments involving membrane nanotubes. Regarding $r$, we have questioned a former demonstration concerning its equality with $\tau$. Finally, the force fluctuation for planar membranes and membrane nanotubes was quantified for the first time.

==> chap4_old.tex <==
\chapter{Fluctuation of forces}
\label{Fluct_TUBE}

As discussed in section~\ref{tube_exp}, nanotubes are
extracted from vesicles by applying point forces.
In the last chapter, we have described a popular method for pulling nanotubes, which consists in attaching a glass bead to the membrane and displacing the bead with a laser.
The advantage of this method is that one can deduce with precision the applied
force by measuring the position of the center of the beam and the position of
the bead along the tube's axis (see Fig.~\ref{fig_3_trap}).
By symmetry, the average of the force 
transversal to the tube's axis vanishes.
Accordingly, one measures in general only the force in the direction of the tube's axis, which we will call here $f_z$.
A typical time-sequence of the bead's position along the tube's axis and force $f_z$ can be seen in Fig.~\ref{fig_4_inaba}.

\begin{figure}[H]
\begin{center}
\includegraphics[scale=.3,angle=0]{./figures_Chap4/inaba.eps}
\caption{Extraction and retraction of a nanotube using a glass bead and an optical
  trap~\cite{Inaba_05}. 
The blue line represents the displacement of the glass bead as a function of
time.
The bead was moved in order to elongate the vesicle and create a tube (from
$0$ up to $80 \, \mathrm{s}$), then kept roughly at the same point for $20 \, \mathrm{s}$ and finally
moved in the opposite direction. 
The red line shows the force applied to the bead.
Note that there is a force barrier to form a tube (region before $40 \, \mathrm{s}$), but afterwards, the force does
almost not depend on the length of the tube.}
\label{fig_4_inaba}
\end{center}      
\end{figure}

Here and in the last chapter, we are interested in the equilibrium situation
where the tube's length is kept constant, which corresponds to the region between the dashed lines in Fig.~\ref{fig_4_inaba}.
In this region, the force is roughly a plateau whose average we have studied in the last chapter, obtaining

\begin{equation}
\langle f_z \rangle \simeq 2\pi\sqrt{2\kappa\sigma}\left[1-
\frac{k_\mathrm{B}T}{4\pi^2}\,\frac{\Lambda^2}{\sigma}\right] \, .
\end{equation}

\noindent Interestingly, in Fig.~\ref{fig_4_inaba}, we see that the measures of $f_z$ present a considerable dispersion,
mainly coming from the fluctuations of the bead's position (we cannot see this
fluctuation on the blue curve due to the length scale).
In effect, the bead is subjected to many sources of thermal fluctuations,
such as the fluctuating forces that the solvent applies to the bead, producing a Brownian movement, and the thermal fluctuations of the membrane to which the bead is attached. 

As membrane nanotubes present very soft
Goldstone modes~\cite{Fournier_07a}, the membrane fluctuation is possibly responsible for most of the dispersion, in which case measures of force fluctuation could be used to characterize membranes.
Indeed, in section~\ref{tube_exp}, we have seen that from measures of the average force
$\langle f_z \rangle$, one can deduce the bending rigidity of a membrane.
Likewise, the fluctuation of the force in the direction of the tube's axis, easily accessible with the same experimental setting, could provide supplemental informations.
Accordingly, our aim in this chapter is to study the contribution of the membrane fluctuations to the fluctuation of the force in the direction of the tube's axis, defined through

\begin{eqnarray}
  (\Delta f_z)^2 &=& \langle f_z^2 \rangle - \langle f_z \rangle^2 \, . 
\end{eqnarray}

As in chapter~\ref{TUBE}, we will consider a tube small enough so that we can
consider the vesicle from which it is extracted as a lipid reservoir and neglect volume constraints.
In section~\ref{section_4_param} we remind some important results deduced in the last chapter.
To evaluate $\Delta f_z$, we will use the diagrammatic tools introduced in
chapter~\ref{Fluct_plan}.
We will thus sum-up some properties of these diagrams and write the stress
tensor using them in section~\ref{section_4_diag}.
In section~\ref{section_4_fluct_calcul}, we evaluate $\Delta f_z$.
Finally, we discuss our results in section~\ref{section_4_discussion}.


\section{Some important definitions and results}
\label{section_4_param}

As in chapter~\ref{TUBE}, we shall restrict our attention to deformed tubes
weakly departing from the mean-field cylinder, whose radius is given by

\begin{equation}
  R_0 = \sqrt{\frac{\kappa}{2\sigma}} \, .
\end{equation}

\noindent We will keep the same coordinate system presented in Fig.~\ref{fig_3_param} and the tube's shape will be parametrized by eq.(\ref{eq_3_param}).  

As before, we consider a tube relatively short compared to the vesicle from which it is extracted, so that the vesicle can be treated as a lipid reservoir.
In the case of short tubes, one can also neglect the pressure difference across
the tube's membrane.
The energy is simply given by the Helfrich Hamiltonian, given in eq.(\ref{eq_3_H}) and eq.(\ref{eq_3_h2}).
The corresponding correlation function is given by

\begin{eqnarray}
  G(\rho - \rho', z- z') &=& \langle u(\rho, z) \, u(\rho', z')\rangle \, ,\nonumber\\
 &=& \frac{k_\mathrm{B}T \, R_0}{2\pi \kappa L} \sum_m \sum_{\bar{q}} \frac{e^{\frac{i}{R_0}\left[m(\rho - \rho') + \bar{q}(z -z')\right]}}{(m^2 -1)^2 + \bar{q}^2(\bar{q}^2 + 2 m^2)} \, ,
\end{eqnarray}

\noindent where $m \in \{-M, \cdots, M\}$ and $\bar{q} = 2\pi n R_0/L$, with $n \in \{-N, \cdots, N\}$.
We remind that the upper bounds $N$ and $M$ are given by $M = \Lambda R_0$ and $\bar{q}_\mathrm{max} = 2 \pi N R_0/L = \Lambda R_0$, where $\Lambda = 1/a$ is the high wave-vector cutoff and $a$ is of the order of the membrane thickness.
For tubes whose length is a few times bigger than $R_0$, one can transform the sum over $\bar{q}$ in an integral, yielding

\begin{equation}
 G(\rho - \rho', z- z') =  \frac{k_\mathrm{B}T }{(2\pi)^2 \kappa} \sum_m \int_{-\Lambda R_0}^{\Lambda R_0} \frac{e^{\frac{i}{R_0}\left[m(\rho - \rho') + \bar{q}(z -z')\right]}}{(m^2 -1)^2 + \bar{q}^2(\bar{q}^2 + 2 m^2)} \, .
\end{equation}

The force needed to extract a tube is given by

\begin{equation}
  \bm{f} = \left(\int_0^{2\pi R_0} \Sigma_{rz} \, d\rho\right) \bm{e}_r + \left(\int_0^{2 \pi R_0} \Sigma_{\rho z} \, d\rho \right) \bm{e}_\rho + \left(\int_0^{2 \pi R_0} \Sigma_{zz} \, d\rho \right) \bm{e}_z \, , 
\end{equation}

\noindent where $\Sigma_{rz}$, $\Sigma_{\rho z}$ and

\begin{eqnarray}
  \Sigma_{zz}&=&\sigma\left\{2+u^2+2R_0^2\left[u_\rho^2+\left(2u-1\right)u_{\rho\rho}\right]\right. \nonumber \\
&+&R_0^4 \left. \left[u_{\rho\rho}^2-u_{zz}^2+2u_z\left(u_{zzz}+u_{\rho\rho
z}\right)\right]\right\}
  \label{eq_4_Sigmazz}
\end{eqnarray}

\noindent are the components of the projected stress tensor for quasi-cylindrical geometry derived in section~\ref{section_3_stress}.
As in the last chapter, the subscript $\rho$ (resp. $z$) indicates the derivative with respect to $\rho$ (resp. $z$).
Here we will evaluate the fluctuation of the force in the direction of the tube's axis:

\begin{eqnarray}
  (\Delta f_z)^2 &=& \langle f_z^2 \rangle - \langle f_z \rangle^2 \, , \nonumber\\
  &=& \int_0^{2 \pi R_0} \int_0^{2\pi R_0} \langle \Sigma_{zz}(\rho,z) \Sigma_{zz}(\rho', z) \rangle - \langle \Sigma_{zz} \rangle^2  \, d\rho d\rho' \, .
  \label{eq_4_Deltafz}
\end{eqnarray}

\noindent As in chapter~\ref{Fluct_plan}, the first step is to evaluate the correlation function of the stress tensor over the same section of tube:

\begin{equation}
  C(\rho, \rho') = \langle \Sigma_{zz}(\rho,z) \Sigma_{zz}(\rho', z) \rangle - \langle \Sigma_{zz} \rangle^2 \, .
\end{equation}

\noindent To do so, we will use another time the diagrammatic tools introduced in chapter~\ref{Fluct_plan}.
In the next section, we recall some properties of these diagrams.



\section{Diagrammatic tools}
\label{section_4_diag}

We will use the same notation of section~\ref{section_11_rules}.
Each field $u(\rho,z)$ is represented by a straight line.
The derivatives with respect to $\rho$ are represented by a dot over the field, while a derivative with respect to $z$ is represented by a slash.
An adapted diagrammatic vocabulary is presented in table~\ref{table_4_vocab}. 

\begin{table}[H]
  \begin{center}
\begin{tabular}{|c|c|}
\hline
\red{Usually} & \red{Diagrammatically} \\
\hline
&\\
$u(\rho,z)$ & \diaggd{./figures_Chap4/simple_0.epsi} \\
&\\
\hline
&\\
$u_z(\rho,z)$ & \diaggd{./figures_Chap4/simple_1.epsi} \\
&\\
\hline
&\\
$u_\rho(\rho,z)$ & \diaggd{./figures_Chap4/simple_4.epsi} \\
&\\
\hline
&\\
$u(\rho,z)\, u(\rho,z)$ & \diaggd{./figures_Chap4/champ_0.epsi} \\
&\\
\hline
&\\
$u(\rho, z)\, u(\rho',z')$ & $\diaggd{./figures_Chap4/simple_0.epsi} \diaggd{./figures_Chap4/simple_0.epsi}$ \\
&\\
\hline
\end{tabular}
\label{table_4_vocab}
\caption{Basic {\it translation} rules from the usual notation into diagrams.}  
\end{center}
\end{table}

Averages are performed using Wick's theorem, i. e., by adding all complete contractions of fields.
Each contraction yields a propagator and, as in the case of section~\ref{section_11_rules}, one can pass a derivative from one branch of the propagator to the other by multiplying the diagram's coefficient by $-1$.
For instance, with $\bm{r} = (\rho, z)$ and $\bm{r}' = (\rho',z')$, we have

\begin{eqnarray}
  \left\langle
  \begin{array}{c}
\diaggd{./figures_Chap4/simple_1.epsi}\\
{}^{\bm{r}}
\end{array}
    \begin{array}{c}
\diaggd{./figures_Chap4/simple_4.epsi}\\
{}^{\bm{r'}}
\end{array}
    \right \rangle &=&
\diaggd{./figures_Chap4/reto_3.epsi} \, ,\nonumber \\
&=&
(-1) \times \diaggd{./figures_Chap4/reto_4.epsi} \, ,\nonumber\\
\nonumber \\
&=& (-1) \times \partial_z \partial_\rho  \, [G(\bm{r}' - \bm{r})] \, ,\nonumber \\
\nonumber\\
 &=& \frac{k_\mathrm{B}T \, R_0}{2\pi \kappa L} \sum_m \sum_{\bar{q}} \frac{(i \, m/R_0)(i \, \bar{q}/R_0) \, e^{\frac{i}{R_0}\left[m(\rho - \rho') + \bar{q}(z -z')\right]}}{(m^2 -1)^2 + \bar{q}^2(\bar{q}^2 + 2 m^2)} \, .
\end{eqnarray}

\noindent This time, once the derivatives are grouped, every slash contributes with a factor $i \, \bar{q}/R_0$ and every dot contributes with a factor $i \,  m/R_0$.

In the following section, we will evaluate the propagators between points over the same section of tube, i. e., with $z = z'$.
In this case, as the sum over $\bar{q}$ is symmetrical, an uneven number of slashes over a propagator imply a vanishing contribution.
Typically, we will have

\begin{eqnarray}
  \left\langle
  \begin{array}{c}
\diaggd{./figures_Chap4/champ_7_n1.epsi}\\
{}^{\bm{r}}
\end{array}
    \begin{array}{c}
\diaggd{./figures_Chap4/champ_7_n2.epsi}\\
{}^{\bm{r}'}
\end{array}
    \right \rangle
    &=&
     \begin{array}{c}
\diaggd{./figures_Chap4/wick_n1.epsi}\\
{}^{\bm{r}}
\end{array}
    \begin{array}{c}
\diaggd{./figures_Chap4/wick_n2.epsi}\\
{}^{\bm{r}'}
\end{array}
+
\diaggd{./figures_Chap4/peixe_n11.epsi}
+
\diaggd{./figures_Chap4/peixe_n21.epsi} \, ,\nonumber \\
&=&    
\diaggd{./figures_Chap4/wick_n1_1.epsi}
\diaggd{./figures_Chap4/wick_n1_1.epsi}
+ 
\diaggd{./figures_Chap4/peixe_n1_1.epsi}
+
\diaggd{./figures_Chap4/peixe_n2_1.epsi}\, ,\nonumber\\
\label{eq_4_avediag}
\end{eqnarray}

\noindent which one can readily read by noting the equivalence

\begin{equation}
\diaggd{./figures_Chap4/peixe_n2_1.epsi} = \diaggd{./figures_Chap4/reto_4.epsi} \times \diaggd{./figures_Chap4/reto_4.epsi} \, .
\label{eq_4_peixe}
\end{equation}

\noindent As the number of slashes over these propagators is uneven, the contribution of this diagram vanishes.
The first term of eq.(\ref{eq_4_avediag}) is also composed by diagrams with an uneven number of slashes whose contribution vanishes.
At the end, on has simply

\begin{eqnarray}
  \left\langle
  \begin{array}{c}
\diaggd{./figures_Chap4/champ_7_n1.epsi}\\
{}^{\bm{r}}
\end{array}
    \begin{array}{c}
\diaggd{./figures_Chap4/champ_7_n2.epsi}\\
{}^{\bm{r}'}
\end{array}
    \right \rangle
    &=&
\diaggd{./figures_Chap4/peixe_n1_1.epsi} \, .
\end{eqnarray}

\noindent In the next section, we will re-derive $\langle \Sigma_{zz} \rangle$ in terms of diagrams to get familiar.

\subsection{Getting familiar: re-deriving $\langle \Sigma_{zz} \rangle$}

The component $\Sigma_{zz}$, given in eq.(\ref{eq_4_Sigmazz}), can be written in terms of diagrams as

\begin{eqnarray}
  \sigma^{-1} \, \langle \Sigma_{zz} \rangle &=& 2 + 
\diaggd{./figures_Chap4/champ_0.epsi}
+ 2 R_0^2 \diaggd{./figures_Chap4/champ_4.epsi}
+ 4 R_0^2 \diaggd{./figures_Chap4/champ_12.epsi}
- 2 R_0^2 \diaggd{./figures_Chap4/simple_5.epsi} \nonumber\\
&+& R_0^4 \diaggd{./figures_Chap4/champ_6.epsi}
- R_0^4 \diaggd{./figures_Chap4/champ_5.epsi}
+ 2 R_0^4 \diaggd{./figures_Chap4/champ_1.epsi}
+  2 R_0^4 \diaggd{./figures_Chap4/champ_2.epsi} \, .
\label{eq_4_Sigmadiag}
\end{eqnarray}

\noindent Using Wick's theorem to evaluate the average, we obtain

\begin{eqnarray}
    \sigma^{-1} \, \langle \Sigma_{zz} \rangle &=& 2 + 
\diaggd{./figures_Chap4/wick_0.epsi}
+ 2 R_0^2 \diaggd{./figures_Chap4/wick_3.epsi}
+ 4 R_0^2 \diaggd{./figures_Chap4/wick_14.epsi}\nonumber\\
&+& R_0^4 \diaggd{./figures_Chap4/wick_5.epsi}
- R_0^4 \diaggd{./figures_Chap4/wick_6.epsi}
+ 2 R_0^4 \diaggd{./figures_Chap4/wick_1.epsi}
+  2 R_0^4 \diaggd{./figures_Chap4/wick_15.epsi} \, .
\end{eqnarray}

\noindent Grouping the derivatives, we have

\begin{eqnarray}
    \sigma^{-1} \, \langle \Sigma_{zz} \rangle &=& 2 + 
\diaggd{./figures_Chap4/wick_0_0.epsi}
- 2 R_0^2 \diaggd{./figures_Chap4/wick_7.epsi}
+ 4 R_0^2 \diaggd{./figures_Chap4/wick_7.epsi}\nonumber\\
&+& R_0^4 \diaggd{./figures_Chap4/wick_9.epsi}
- R_0^4 \diaggd{./figures_Chap4/wick_10.epsi}
- 2 R_0^4 \diaggd{./figures_Chap4/wick_10.epsi}
-  2 R_0^4 \diaggd{./figures_Chap4/wick_11.epsi} \, , \nonumber\\
\nonumber \\
&=& 2 + 
\diaggd{./figures_Chap4/wick_0_0.epsi}
+ 2 R_0^2 \diaggd{./figures_Chap4/wick_7.epsi}
+ R_0^4 \diaggd{./figures_Chap4/wick_9.epsi}
- 3 R_0^4 \diaggd{./figures_Chap4/wick_10.epsi}
-  2 R_0^4 \diaggd{./figures_Chap4/wick_11.epsi} \, . \nonumber\\
\label{eq_4_aveSigma}
\end{eqnarray}

\noindent Just to get familiar, let's read eq.(\ref{eq_4_aveSigma}):

\begin{eqnarray}
  \langle \Sigma_{zz} \rangle &=& 2 \sigma  + \sigma \frac{k_\mathrm{B} T \, R_0}{2 \pi \kappa L} \sum_m \sum_{\bar{q}} \frac{1 + 2(i \, m)^2 + (i \, m)^4 - 3 (i \, \bar{q})^4 -2 (i \, m)^2(i \, \bar{q})^2}{(m^2 - 1)^2 + \bar{q}^2(\bar{q}^2 + 2 m^2)} \, , \nonumber\\
  &=& 2 \sigma  + \frac{k_\mathrm{B} T }{4 \pi R_0 L} \sum_m \sum_{\bar{q}} \frac{(1-m^2)^2 - \bar{q}^2(3 \bar{q}^2 + 2 m^2)}{(m^2 - 1)^2 + \bar{q}^2(\bar{q}^2 + 2 m^2)} \, ,
\end{eqnarray}

\noindent which coincides, as it should, with eq.(\ref{eq_3_Sigmamoy}).


\section{Evaluation of the fluctuation of the force}
\label{section_4_fluct_calcul}

Here we evaluate $\Delta f_z$.
We start by evaluating the correlation function of the component $\Sigma_{zz}$ of the stress tensor.
In section~\ref{section_4_Df}, we integrate twice this correlation and obtain $\Delta f_z$.
There, we discuss also some approximations in order to obtain a simple analytical expression.
Finally, we conclude by a short discussion on the validity of our final result in section~\ref{section_4_validity}.

\subsection{Correlation of $\Sigma_{zz}$}
\label{subsection_4_corr}

Here we will evaluate the correlation function

\begin{equation}
  C(\rho, \rho') = \langle \Sigma_{zz}(\rho,z) \Sigma_{zz}(\rho', z) \rangle - \langle \Sigma_{zz} \rangle^2 \, .
\end{equation}

\noindent From eq.(\ref{eq_4_Sigmadiag}), using Wick's Theorem and the rules presented in section~\ref{section_4_diag}, we obtain

\begin{eqnarray}
\sigma^{-2} \, C(\rho, \rho') &=&
2 \diagH{./figures_Chap4/diag.eps}
+ 8 R_0^2 \diagH{./figures_Chap4/diagpop.eps}
+ 16 R_0^2 \diagH{./figures_Chap4/diagppo.eps}
+ 28 R_0^4 \diagH{./figures_Chap4/diagppopp.eps} \nonumber\\
&+& 32 R_0^4 \diagH{./figures_Chap4/diagpppop.eps}
+ 16 R_0^4 \diagH{./figures_Chap4/diagppppo.eps}
- 4 R_0^4 \diagH{./figures_Chap4/diagttott.eps}
+ 8 R_0^6 \diagH{./figures_Chap4/diagpppoppp.eps} \nonumber\\
&-&8 R_0^6 \diagH{./figures_Chap4/diagttpottp.eps}
+ 16 R_0^6 \diagH{./figures_Chap4/diagppppopp.eps}
- 16 R_0^6 \diagH{./figures_Chap4/diagttppott.eps}
+2 R_0^8 \diagH{./figures_Chap4/diagppppopppp.eps}\nonumber\\
&+& 6 R_0^8 \diagH{./figures_Chap4/diagttttotttt.eps} 
+8 R_0^8 \diagH{./figures_Chap4/diagttppotttt.eps}
+4 R_0^8 \diagH{./figures_Chap4/diagttttttott.eps}
+ 4 R_0^8 \diagH{./figures_Chap4/diagttppppott.eps} \nonumber\\
&+& 8 R_0^8 \diagH{./figures_Chap4/diagttttppott.eps}
+4 R_0^4 \diagH{./figures_Chap4/diagpppp.eps} \, .
\label{eq_4_fluctdiag}
\end{eqnarray}

\noindent Note that all the terms involving diagrams of the kind $\diaggd{./figures_Chap4/wick_0_0.epsi}$ vanish.
Explicitly, we obtain

\begin{eqnarray}
  C(\rho, \rho') &=& \left(\frac{k_B T}{4\pi R_0 L} \right)^2 \sum_{m,\bar{q}} \sum_{n,\bar{k}} f_{n,m,\bar{q},\bar{k}} \, e^{i R_0^{-1} (m+n)(\rho - \rho')} \nonumber \\
  &+& 2 \, \frac{\kappa}{R_0^2} \left(\frac{k_\mathrm{B} T}{4\pi R_0 L}\right) \sum_{m,
    \bar{q}} \frac{m^4 \, e^{iR_0^{-1} m(\rho - \rho')}}{(m^2 -1)^2 +
    \bar{q}^2(\bar{q}^2 + 2 m^2)} \, ,
\label{eq_4_C}
\end{eqnarray}

\noindent where $f_{n,m,\bar{q}, \bar{q}}$ is a complicated coefficient
depending on $m$, $n$, $\bar{q}$ and $\bar{k}$:

\begin{equation}
f_{n,m,\bar{q},\bar{k}} = \frac{g_{n,m,\bar{q}, \bar{k}}}{\left[(m^2 -1)^2 +
    \bar{q}^2(\bar{q}^2 + 2 m^2)\right]\left[(n^2 -1)^2 + \bar{k}^2(\bar{k}^2
    + 2 n^2)\right]} \, ,
\end{equation}

\noindent with

\begin{eqnarray}
g_{n,m,\bar{q},\bar{k}} &=& 2 - 16\,  m^2 + 16 \, m^4 - 8 \, m\, n + 32 \, m^3
\, n + 28\, m^2 \, n^2 - 16 \, m^4 \, n^2 \nonumber\\
&-& 8 \, m^3 \, n^3 + 2 \, m^4\, n^4 - 4 \, \bar{q}^2 \, \bar{k}^2 + 16 \, m^2
\, \bar{q}^2 \, \bar{k}^2 + 8 \, m^2 \, \bar{q}^2 \, \bar{k}^4 \nonumber\\
&+& 4 \, m^4\, \bar{q}^2 \bar{k}^2 + 8 \, m\, n \, \bar{q}^2 \, \bar{k}^2 + 6
\, \bar{q}^4 \, \bar{k}^4 + 8 \, m^2 \, \bar{q}^4 \, \bar{k}^2 + 4 \,
\bar{q}^6 \, \bar{k}^2 \, .
\end{eqnarray}

\noindent The second term of eq.(\ref{eq_4_C}) is the contribution given by the last diagram of eq.(\ref{eq_4_fluctdiag}).
As expected, the correlation depends only on $\rho - \rho'$.
In Fig.~\ref{fig_4_correl}, we show the behavior of the correlation normalized by it's value at $\rho = 0$ for two different tubes with the same length, bending rigidity and wave-length cut-off.

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.6\columnwidth]{./figures_Chap4/correl.eps}
\caption{Correlation function of the component $\Sigma_{zz}$ of the stress tensor normalized by it's value at $\rho = 0$ as a function of $\rho/R_0$.
  In both curves, we considered tubes of length $500 \, \mathrm{nm}$ and bending rigidity $\kappa = 50 \, k_\mathrm{B}T$.
  We have chosen $\Lambda^{-1} = 5 \,  \mathrm{nm}$ as the value of the microscopical cut-off.
  The blue curve stands for a thin tube with $R_0 = 30 \, \mathrm{nm}$, while the red curve stands for a tube with $R_0 = 100 \, \mathrm{nm}$.}
\label{fig_4_correl}
\end{center}      
\end{figure}

First of all, we note that even though the stress tensor correlation decreases with the distance, we have no more the fast decay found in the case of planar membranes (see section~\ref{section_11_corr}).
The function $C(\rho)$ presents an oscillating behavior that takes place over a characteristic length $a$, where $a = \Lambda^{-1}$.
These oscillations remain non-negligible throughout the whole section of the tube, indicating that the stress tensor is correlated all over the length of a cross section.
This is a signature of the fact that the fluctuations in the shape of membrane tubes are themselves correlated over a cross section, whatever the tube's radius \cite{Fournier_07a}.

To characterize better how the stress tensor correlation decreases, we have plotted the absolute value of the extrema of the oscillations of the red curve as a function of $\rho/R_0$ in a log-log scale (see Fig.~\ref{fig_4_power_law}).
This curve seems to indicate that the amplitude of the oscillations decay with a power law, which is a characteristic sign of long-range correlations.

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.6\columnwidth]{./figures_Chap4/power_law.eps}
\caption{The red dots represent the absolute value of the extrema of the red curve in Fig.~\ref{fig_4_correl} as a function of $\rho/R_0$.
The blue curve is proportional to $x^{-1}$.}
\label{fig_4_power_law}
\end{center}      
\end{figure}

Finally, we have compared the contributions of the first and the second terms of eq.(\ref{eq_4_C}) to the total stress tensor correlation.
As one can see in Fig.~\ref{fig_4_comp_a} and in Fig.~\ref{fig_4_comp_b}, in general, both contributions are oscillating and non-negligible at this point.
In the following, however, we will see that only the first term of eq.(\ref{eq_4_C}), represented by green curves in these figures, is important to evaluate $\Delta f_z$.

\begin{figure}[H]
\begin{center}
\subfigure[Tube with $R_0 = 30 \, \mathrm{nm}$.]{
\includegraphics[width=0.45\columnwidth]{./figures_Chap4/comp_30.eps}
\label{fig_4_comp_a}
}  
\subfigure[Tube with $R_0 = 100 \, \mathrm{nm}$.]{ 
  \includegraphics[width=0.45\columnwidth]{./figures_Chap4/comp_100.eps}
  \label{fig_4_comp_b}
}
\caption{Contribution of the first term of eq.(\ref{eq_4_C}) to the stress tensor correlation (green curve) compared to the contribution of the second term of this equation (violet curve).
In both cases, we have considered tubes with length $500 \, \mathrm{nm}$, $\kappa = 50 \, k_\mathrm{B}T$ and $\Lambda^{-1} = 5 \, \mathrm{nm}$.}
\end{center}      
\end{figure}

\subsection{Force fluctuation $\Delta f_z$}
\label{section_4_Df}

As we have seen in eq.(\ref{eq_4_Deltafz}), the force fluctuation is given by

\begin{equation}
  (\Delta f_z)^2 = \int_0^{2\pi R_0} \int_0^{2\pi R_0} C(\rho, \rho') \, d\rho d\rho' \, .
  \label{eq_4_deltafz}
\end{equation}

\noindent Performing the changing of variable $\rho'' = \rho - \rho'$, eq.(\ref{eq_4_deltafz}) becomes

\begin{equation}
  (\Delta f_z)^2 = \int_0^{2\pi R_0} \int_{-\rho'}^{2\pi R_0 - \rho'} C(\rho'', 0) \, d\rho'' d\rho \, .
\end{equation}

\noindent As the function $C(\rho'', 0)$ is periodic with period $2 \pi R_0$, this integral is equivalent to

\begin{equation}
  (\Delta f_z)^2 = 2\pi R_0  \int_0^{2\pi R_0} C(\rho'', 0) \, d\rho'' \, .
\end{equation}

\noindent Using the fact that

\begin{equation}
  \int_0^{2\pi R_0} e^{i R_0^{-1} (m + n)\rho''} \, d\rho'' = 2\pi R_0 \, \delta_{n, -m} \, ,
\end{equation}

\noindent we obtain

\begin{eqnarray}
  (\Delta f_z)^2 &=& (2 \pi R_0)^2 \left(\frac{k_B T}{4\pi R_0 L} \right)^2 \sum_{m,\bar{q}} \sum_{\bar{k}} f_{-m,m,\bar{q},\bar{k}}  \, ,\nonumber \\
  &=& \left(\frac{k_\mathrm{B} T}{2 L} \right)^2 \sum_{m,\bar{q}} \sum_{\bar{k}} \frac{2(m^2-1)^4+4\bar{k}^2 \bar{q}^2 \left[\bar{k}^4-1+2m^2\left(1+2\bar{k}^2\right)+m^4\right]+6\bar{k}^4\bar{q}^4}{\left[(m^2-1)^2+\bar{q}^2(\bar{q}^2+2m^2)\right]\,\left[(m^2-1)^2+\bar{k}^2(\bar{k}^2+2m^2)\right]} \, . \nonumber\\
\end{eqnarray}

\noindent Note that the contribution of the last term of eq.(\ref{eq_4_C})
vanishes after integration.

\subsubsection{Long tubes}

For the case of $L > R_0$,
we can substitute the sums over $\bar{q}$ and over $\bar{k}$ by integrals, yielding

\begin{equation}
  \begin{split}
&(\Delta f_z)^2= \\
&\left(\frac{k_\mathrm{B}T}{4\pi R_0}\right)^2\!
\sum_{m=-M}^M \int_{-\Lambda R}^{\Lambda R_0} \int_{-\Lambda R_0}^{\Lambda R}
\frac{
2(m^2-1)^4
+4\bar k^2\bar q^2
\left[
\bar k^4-1+2m^2\left(1+2\bar k^2\right)+m^4
\right]+6\bar k^4\bar q^4
}{
\left[
(m^2-1)^2+\bar q^2(\bar q^2+2m^2)
\right]\,\left[
(m^2-1)^2+\bar k^2(\bar k^2+2m^2)
\right]
} \, 
d\bar q\,
d\bar k \, .
\end{split}
  \label{eq_4_Deltafzcalcul}
\end{equation}

\noindent Taking into account the fact that
eq.(\ref{eq_4_Deltafzcalcul}) depends only on $|m|$, it can be rewritten as

\begin{equation}
(\Delta f_z)^2= 
\left(\frac{k_\mathrm{B}T}{4\pi R_0}\right)^2\! \left(T_0 + 2 \, T_1 + 2 \,
  \sum_{m=2}^M T_m\right) \,,
\label{eq_4_D}
\end{equation} 

\noindent with

\begin{equation}
T_0 = \int_{-\Lambda R}^{\Lambda R} \int_{-\Lambda R}^{\Lambda R}
\frac{2 \bar{q}^4 \bar{k}^4 \left(\bar{q}^2 + \bar{k}^2\right) + \left(1 -
    \bar{q}^2 \bar{k}^2 \right)^2}{\left(1 + \bar{q}^4 \right)\left(1 +
    \bar{k}^4 \right)
} \, 
d\bar q\,
d\bar k \, ,
\label{eq_4_T0}
\end{equation}

\begin{equation}
T_1 = \int_{-\Lambda R}^{\Lambda R} \int_{-\Lambda R}^{\Lambda R}
\frac{8 + 4 \bar{k}^4 + 2 \bar{k}^2 \left(8 + 3 \bar{q}^2\right)}{\left( 2 +
    \bar{q}^2 \right)\left(2 + \bar{k}^2 \right)} \, 
d\bar q\,
d\bar k \, ,
\label{eq_4_T1}
\end{equation}

\noindent and

\begin{equation}
T_m = \int_{-\Lambda R}^{\Lambda R} \int_{-\Lambda R}^{\Lambda R}
\frac{
2(m^2-1)^4
+4\bar k^2\bar q^2
\left[
\bar k^4-1+2m^2\left(1+2\bar k^2\right)+m^4
\right]+6\bar k^4\bar q^4
}{
\left[
(m^2-1)^2+\bar q^2(\bar q^2+2m^2)
\right]\,\left[
(m^2-1)^2+\bar k^2(\bar k^2+2m^2)
\right]
} \, 
d\bar q\,
d\bar k \, .
\label{eq_4_Tm}
\end{equation}
 
\noindent Both integrals over $\bar{q}$ and over $\bar{k}$ in
eq.(\ref{eq_4_T0}), eq.(\ref{eq_4_T1}) and eq.(\ref{eq_4_Tm}) can be performed
analytically.
One can compare the contributions of some modes in Fig.~\ref{fig_4_modes}.
Not surprisingly, the modes $|m|=1 $, which are extremely soft~\cite{Fournier_07}, give a greater contribution to the force.


\begin{figure}[H]
\begin{center}
\includegraphics[width = 0.7\columnwidth]{./figures_Chap4/modes1.eps}
\caption{Contribution of some modes to the force fluctuation in units of
  $[k_\mathrm{B} T/(4 \pi R_0)]^{2}$ as a function of the radius of the tube
  in units of the microscopical cutoff $a = \Lambda^{-1}$.
The dashed line corresponds to the contribution of the modes with $m=0$, the
red line corresponds to the soft modes with $|m|=1$, and the blue and green
lines correspond to $|m| = 2$ and $|m| = 3$, respectively.
We see that the Goldstone modes give indeed a greater contribution to the
force fluctuation.}
\label{fig_4_modes}
\end{center}      
\end{figure}

\noindent In Fig.~\ref{fig_4_porcent}, we show the percent contribution of
these soft modes to the total fluctuation.
In agreement with the curves of Fig.~\ref{fig_4_modes}, the soft modes are responsible for more than one third of the force fluctuation.

\begin{figure}[H]
\begin{center}
\includegraphics[width = 0.7\columnwidth]{./figures_Chap4/Procent.eps}
\caption{Percent contribution of the soft modes ($|m| = 1$) to the total
  force fluctuation.}
\label{fig_4_porcent}
\end{center}      
\end{figure}

\subsubsection{Approximations and an analytical formula for $\Delta f_z$}

In order to obtain a simple analytical expression to the force fluctuation, we
consider the limit for relatively thick tubes, with $\Lambda \, R_0 > 6$.
Considering $a = \Lambda^{-1} = 5 \, \mathrm{nm}$, this corresponds to tubes
with an radius $R_0 > 30 \, \mathrm{nm}$, which is currently observed in experiments.  
In this limit, we have

\begin{equation}
T_0 \approx \frac{2 \sqrt{2} \pi}{3} \, (\Lambda \, R_0)^3 \, ,
\end{equation}

\begin{equation}
T_1 \approx \frac{4\sqrt{2} \pi}{3} \, (\Lambda \, R_0)^3 \, ,
\end{equation}

\noindent and 

\begin{eqnarray}
T_m \approx 24 (\Lambda \, R_0)^2 + \frac{8}{3m}\left[(\Lambda \,
    R_0)^3 - 21 m^2 (\Lambda \, R_0) + 12 m^3 \arctan\left(\frac{\Lambda \,
        R_0}{m}\right) \right] \arctan\left(\frac{\Lambda \, R_0}{m} \right)
  \, . \nonumber\\
\end{eqnarray}

\noindent In this case, we can approximate the sum over $m$ in
eq.(\ref{eq_4_D}) by an integral:

\begin{equation}
\sum_{m=2}^{M} T_m \approx \int_2^{\Lambda \, R_0} T_m \, dm \simeq \frac{2 \sqrt{2} \pi}{3} \, (\Lambda \, R_0)^3 \, + \frac{4
  \pi}{3} \, (\Lambda \, R_0)^3 \, \ln(\Lambda \, R_0) \, .
\end{equation}

\noindent Finally, we obtain

\begin{equation}
\left(\Delta f_z\right)^2 \simeq \frac{(k_\mathrm{B}T)^2 \, R_0\, \Lambda^3}{6\pi} \left[\frac{5}{2} + \ln\left(\Lambda \, R_0\right)\right] \, .
\label{eq_4_Dfapprox}
\end{equation}

\noindent We discuss the quality of this approximation and its meaning in section~\ref{section_4_discussion}. 

\subsection{Discussion on the validity of this result}
\label{section_4_validity}

Here we remind the conditions of validity of eq.(\ref{eq_4_D}).
First, as we consider only deformations up to order two, this result corresponds actually to the first term in a series expansion of the form

\begin{equation}
  (\Delta f_z)^2 = f_0^2 \left[\left(\frac{k_\mathrm{B} T}{\kappa}\right)^2 \, g_1(\Lambda \, R_0) + \left(\frac{k_\mathrm{B} T}{\kappa}\right)^3 \, g_2(\Lambda \, R_0) + \cdots \right] \, .
\end{equation}

\noindent Secondly, eq.(\ref{eq_4_D}) is valid for tubes relatively long, i. e., whose length is bigger than the radius, but still small compared to the radius of the vesicle from which it is extracted.
The simplified eq.(\ref{eq_4_Dfapprox}) is a good approximation under the supplemental condition $\Lambda \, R_0 > 6$.

Finally, let us comment on the influence of the boundary conditions.
Differently from the case of the average force, there is no conservation principle for $\Delta f_z$.
Here, we have calculated $\Delta f_z$ assuming periodic boundary conditions, or equivalently,
through an arbitrary section in the middle of a long enough tube.
The actual value of $\Delta f_z$ at the extremity of a tubule with specific
boundary conditions might be somewhat different.
Note also that we have
only calculated the fluctuation of the component of the force which is
parallel to the tube axis.

\section{Discussion and consequences for experiments}
\label{section_4_discussion}

First of all, let us discuss on the dependence of $\Delta f_z$ on $R_0$.
From eq.(\ref{eq_4_Dfapprox}), we have

\begin{equation}
  \Delta f_z \propto \sqrt{\frac{R_0}{a}} \left(\frac{k_\mathrm{B} T}{a} \right) \times \sqrt{\ln\left(\frac{R_0}{a}\right)} \, ,
\end{equation}

\noindent with $a = \Lambda^{-1}$ of the order of the membrane thickness.
The first term reminds the result obtained in chapter~\ref{Fluct_plan}.
There, we have seen that for planar membranes, the correlation of the stress tensor decreases over a very short length, whatever the membrane tension or rigidity.
One could thus consider that a piece of membrane was a composition of uncorrelated patches of size $\approx a$ and use the Central Limit Theorem to obtain the force fluctuation.
Differently, here we see that the size of the patch depends on the membrane rigidity and tension through $R_0$.
Moreover, the force fluctuation of tubes has a logarithmic correction to the planar force fluctuation.
This correction can be explained by the fact that the correlation of the stress tensor in membrane nanotubes decreases in a power law, as we have shown in section~\ref{subsection_4_corr}.

In Fig.~\ref{fig_4_fluctR}, we show $\Delta f_z$ as a function on $R_0$.
The exact curve for long tubes given in eq.(\ref{eq_4_D}) is indicated by circles, while the approximation given in eq.(\ref{eq_4_Dfapprox}) corresponds to the solid lines.
We can see the good quality of the approximation.
For a given value of $\Lambda$, $\Delta f_z$ does not vary much over the experimental range of $R_0$.
On the contrary, it depends strongly on the value of the cutoff $\Lambda$. 
These values of $\Delta f_z$ seem compatible with the force fluctuation curves shown in Fig.~\ref{fig_4_inaba}, in \cite{Koster_05} and \cite{Cuvelier_05}.
For an accurate comparison, however,
time-resolved measurements should be performed and the Brownian force on
the pulling bead should be taken into account.

\begin{figure}[H]
\begin{center}
\includegraphics[width = 0.65\columnwidth]{./figures_Chap4/fluctR.eps}
\caption{Force fluctuation as a function of the tube's radius.
The solid lines correspond to the approximation given in eq.(\ref{eq_4_Dfapprox}).
The curves for $\Lambda \, a = 2, \, 1 \, ,0.5$ are shown, respectively, in blue, red and green.
The circles stand for the exact numerical sum (eq.(\ref{eq_4_D})).
Remark the good quality of the approximation.
In this plot, we have considered $k_\mathrm{B} T = 4 \times 10^{-21} \, \mathrm{J}$ and $a = 5 \, \mathrm{nm}$.}
\label{fig_4_fluctR}
\end{center}      
\end{figure}

\noindent We can also remark that $\Delta f_z$ is rather small compared to the force $f_z$ needed to extract a tube, despite the presence of soft Goldstone modes.
In Fig.~\ref{fig_4_flucttau}, we show the curve of the force $f_z$ as a function of $\tau$ already presented in Fig.~\ref{fig_3_fentau} and we add the curve of $\Delta f_z$ for comparison.
We find $\Delta f_z$ comparable to $f_z$ for
$\tau<10^{-6}\mathrm{J/m}^2$, but quite negligible for
$\tau>10^{-5}\mathrm{J/m}^2$.
Sadly, we can see explicitly that $\Delta f_z$ does almost not depend on the tension of the membrane.
Consequently, $\Delta f_z$ seems to be a not very useful tool to characterize a  membrane, since it is almost constant. 

\begin{figure}[H]
\centerline{\includegraphics[width=.65\columnwidth]{./figures_Chap4/fentau_new1.eps}}
\caption{
Average force $f$ (in red) and it's fluctuation $\Delta f_z$ (in blue) as a function of
the effectively applied mechanical tension $\tau$.
The
parameters used are $\Lambda \, a=1$ with $a\simeq5\, \mathrm{nm}$,
$k_BT\simeq4\times10^{-21}\, \mathrm{J}$ and $\kappa\simeq50\,k_BT$.  
}
\label{fig_4_flucttau}
\end{figure}

\section{In a nutshell}

In this chapter we have examined the possibility of using the fluctuation of the force along a membrane tube's axis $\Delta f_z$ as a tool to characterize membranes since it is known that membrane nanotubes present very soft modes.
For a weakly fluctuating tube whose length $L$ respects $R_\mathrm{ves} \geq L > R_0$, where $R_\mathrm{ves}$ is the radius of the vesicle from with the tube is pulled and $R_0$ is the mean-field radius of the tube, we obtained

\begin{equation}
\left(\Delta f_z\right)^2 \simeq \frac{(k_\mathrm{B}T)^2 \, R_0\, \Lambda^3}{6\pi} \left[\frac{5}{2} + \ln\left(\Lambda \, R_0\right)\right] \, ,
\end{equation}

\noindent where $\Lambda^{-1} = a$, with $a$ of the order of the membrane thickness.
Numerically, for $a \approx 5 \, \mathrm{nm}$, we have found $\Delta f_z \approx 1 \mathrm{pN}$, in agreement with experimental data.
This expression is extremely sensitive to the value of $\Lambda$, whereas it does almost not depend on the radius or on the tension.
Accordingly, $\Delta f_z$ seems of little utility to membrane characterization.
Interestingly, however, one has 

\begin{equation}
  \Delta f_z \propto \sqrt{\frac{R_0}{a}} \left(\frac{k_\mathrm{B} T}{a} \right) \times \sqrt{\ln\left(\frac{R_0}{a}\right)} \, .
\end{equation}

\noindent The logarithmic correction is a signature of the long-range correlations present in the tubes.  

